On the Performance Analysis of Underlay Cognitive Radio Systems: A Deployment Perspective

We study the performance of cognitive Underlay System (US) that employ power control mechanism at the Secondary Transmitter (ST) from a deployment perspective. Existing baseline models considered for performance analysis either assume the knowledge of involved channels at the ST or retrieve this information by means of a band manager or a feedback channel, however, such situations rarely exist in practice. Motivated by this fact, we propose a novel approach that incorporates estimation of the involved channels at the ST, in order to characterize the performance of the US in terms of interference power received at the primary receiver and throughput at the secondary receiver (or \textit{secondary throughput}). Moreover, we apply an outage constraint that captures the impact of imperfect channel knowledge, particularly on the uncertain interference. Besides this, we employ a transmit power constraint at the ST to classify the operation of the US in terms of an interference-limited regime and a power-limited regime. In addition, we characterize the expressions of the uncertain interference and the secondary throughput for the case where the involved channels encounter Nakagami-$m$ fading. Finally, we investigate a fundamental tradeoff between the estimation time and the secondary throughput depicting an optimized performance of the US.

==> figures/fig_CDF_Cs_diff_SNR_p2.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{fig_CDF_Cs_diff_SNR_p2}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           06-Jun-2016 06:03:24
% eps bounding box:     16 cm x 12 cm
% comment:              
%
%\begin{psfrags}%
%\psfragscanon%
%
% text strings:
\psfrag{s05}[t][t]{\fontsize{8}{12}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\eca$ [bits/sec/Hz]\end{tabular}}%
\psfrag{s06}[b][b]{\fontsize{8}{12}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}CDF\end{tabular}}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[l][l]{\fontsize{8}{12}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}Simulated}%
\psfrag{s13}[l][l]{\fontsize{8}{12}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}Theoretical}%
\psfrag{s14}[l][l]{\fontsize{8}{12}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}Simulated}%
%
% axes font properties:
\fontsize{8}{12}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{3}%
\psfrag{x02}[t][t]{3.5}%
\psfrag{x03}[t][t]{4}%
\psfrag{x04}[t][t]{4.5}%
\psfrag{x05}[t][t]{5}%
\psfrag{x06}[t][t]{5.5}%
\psfrag{x07}[t][t]{6}%
\psfrag{x08}[t][t]{6.5}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.1}%
\psfrag{v03}[r][r]{0.2}%
\psfrag{v04}[r][r]{0.3}%
\psfrag{v05}[r][r]{0.4}%
\psfrag{v06}[r][r]{0.5}%
\psfrag{v07}[r][r]{0.6}%
\psfrag{v08}[r][r]{0.7}%
\psfrag{v09}[r][r]{0.8}%
\psfrag{v10}[r][r]{0.9}%
%
% Figure:
%\resizebox{8cm}{!}{\includegraphics{fig_CDF_Cs_diff_SNR_p2.eps}}%
%\end{psfrags}%
%
% End fig_CDF_Cs_diff_SNR_p2.tex


==> figures/fig_opt_est_time_vs_SNR_fading.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{fig_opt_est_time_vs_SNR_fading}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           19-Aug-2015 14:07:04
% eps bounding box:     16 cm x 12 cm
% comment:              
%
%\begin{psfrags}%
%\psfragscanon%
%
% text strings:
\psfrag{s03}[b][b]{\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\ttau$ [ms]\end{tabular}}%
\psfrag{s04}[t][t]{\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\gamma$ [dB]\end{tabular}}%
%
% axes font properties:
\fontsize{9}{13.5}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{-15}%
\psfrag{x02}[t][t]{-10}%
\psfrag{x03}[t][t]{-5}%
\psfrag{x04}[t][t]{0}%
\psfrag{x05}[t][t]{5}%
\psfrag{x06}[t][t]{10}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.5}%
\psfrag{v03}[r][r]{1}%
\psfrag{v04}[r][r]{1.5}%
\psfrag{v05}[r][r]{2}%
%
% Figure:
%\resizebox{8cm}{!}{\includegraphics{fig_opt_est_time_vs_SNR_fading.eps}}%
%\end{psfrags}%
%
% End fig_opt_est_time_vs_SNR_fading.tex


==> figures/fig_opt_thr_vs_SNR_AWGN.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{fig_opt_thr_vs_SNR_AWGN}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           13-Dec-2015 21:43:34
% eps bounding box:     16 cm x 12 cm
% comment:              
%
%\begin{psfrags}%
%\psfragscanon%
%
% text strings:
\psfrag{s08}[b][b]{\fontsize{8.5}{12.75}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\rs(\ttau)$ [bits/sec/Hz]\end{tabular}}%
\psfrag{s09}[t][t]{\fontsize{8.5}{12.75}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\gamma$ [dB]\end{tabular}}%
\psfrag{s13}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s14}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s15}[l][l]{\fontsize{8.5}{12.75}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}EM, $\opc = 0.1$}%
\psfrag{s16}[l][l]{\fontsize{8.5}{12.75}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}IM}%
\psfrag{s17}[l][l]{\fontsize{8.5}{12.75}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}EM, $\opc = 0.01$}%
\psfrag{s18}[l][l]{\fontsize{8.5}{12.75}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}EM, $\opc = 0.1$}%
\psfrag{s19}[b][b]{\fontsize{8.5}{12.75}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Zoom\end{tabular}}%
%
% axes font properties:
\fontsize{8.5}{12.75}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{-1}%
\psfrag{x02}[t][t]{-0.8}%
\psfrag{x03}[t][t]{-0.6}%
\psfrag{x04}[t][t]{-0.4}%
\psfrag{x05}[t][t]{-20}%
\psfrag{x06}[t][t]{-15}%
\psfrag{x07}[t][t]{-10}%
\psfrag{x08}[t][t]{-5}%
\psfrag{x09}[t][t]{0}%
\psfrag{x10}[t][t]{5}%
\psfrag{x11}[t][t]{10}%
%
% yticklabels:
\psfrag{v01}[r][r]{2.5}%
\psfrag{v02}[r][r]{2.6}%
\psfrag{v03}[r][r]{2.7}%
\psfrag{v04}[r][r]{2.8}%
\psfrag{v05}[r][r]{0}%
\psfrag{v06}[r][r]{1}%
\psfrag{v07}[r][r]{2}%
\psfrag{v08}[r][r]{3}%
\psfrag{v09}[r][r]{4}%
\psfrag{v10}[r][r]{5}%
\psfrag{v11}[r][r]{6}%
\psfrag{v12}[r][r]{7}%
\psfrag{v13}[r][r]{8}%
\psfrag{v14}[r][r]{9}%
%
% Figure:
%\resizebox{8cm}{!}{\includegraphics{fig_opt_thr_vs_SNR_AWGN.eps}}%
%\end{psfrags}%
%
% End fig_opt_thr_vs_SNR_AWGN.tex


==> figures/fig_opt_thr_vs_SNR_fading.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{fig_opt_thr_vs_SNR_fading}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           20-Dec-2015 09:26:34
% eps bounding box:     16 cm x 12 cm
% comment:              
%
%\begin{psfrags}%
%\psfragscanon%
%
% text strings:
\psfrag{s05}[b][b]{\fontsize{8.5}{12.75}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\rs(\ttau)$ [bits/sec/Hz]\end{tabular}}%
\psfrag{s06}[t][t]{\fontsize{8.5}{12.75}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\gamma$ [dB]\end{tabular}}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[l][l]{\fontsize{8.5}{12.75}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}Lemma 2}%
\psfrag{s13}[l][l]{\fontsize{8.5}{12.75}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}IM}%
\psfrag{s14}[l][l]{\fontsize{8.5}{12.75}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}EM}%
\psfrag{s15}[l][l]{\fontsize{8.5}{12.75}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}Lemma 2}%
%
% axes font properties:
\fontsize{8.5}{12.75}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{-20}%
\psfrag{x02}[t][t]{-15}%
\psfrag{x03}[t][t]{-10}%
\psfrag{x04}[t][t]{-5}%
\psfrag{x05}[t][t]{0}%
\psfrag{x06}[t][t]{5}%
\psfrag{x07}[t][t]{10}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{1}%
\psfrag{v03}[r][r]{2}%
\psfrag{v04}[r][r]{3}%
\psfrag{v05}[r][r]{4}%
\psfrag{v06}[r][r]{5}%
\psfrag{v07}[r][r]{6}%
\psfrag{v08}[r][r]{7}%
%
% Figure:
%\resizebox{8cm}{!}{\includegraphics{fig_opt_thr_vs_SNR_fading.eps}}%
%\end{psfrags}%
%
% End fig_opt_thr_vs_SNR_fading.tex

